DIRECT-3D: Learning Direct Text-to-3D Generation on Massive Noisy 3D Data

We present DIRECT-3D, a diffusion-based 3D generative model for creating high-quality 3D assets (represented by Neural Radiance Fields) from text prompts. Unlike recent 3D generative models that rely on clean and well-aligned 3D data, limiting them to single or few-class generation, our model is directly trained on extensive noisy and unaligned `in-the-wild' 3D assets, mitigating the key challenge (i.e., data scarcity) in large-scale 3D generation. In particular, DIRECT-3D is a tri-plane diffusion model that integrates two innovations: 1) A novel learning framework where noisy data are filtered and aligned automatically during the training process. Specifically, after an initial warm-up phase using a small set of clean data, an iterative optimization is introduced in the diffusion process to explicitly estimate the 3D pose of objects and select beneficial data based on conditional density. 2) An efficient 3D representation that is achieved by disentangling object geometry and color features with two separate conditional diffusion models that are optimized hierarchically. Given a prompt input, our model generates high-quality, high-resolution, realistic, and complex 3D objects with accurate geometric details in seconds. We achieve state-of-the-art performance in both single-class generation and text-to-3D generation. We also demonstrate that DIRECT-3D can serve as a useful 3D geometric prior of objects, for example to alleviate the well-known Janus problem in 2D-lifting methods such as DreamFusion. The code and models are available for research purposes at: https://github.com/qihao067/direct3d.

==> tab/abl_prompt.tex <==
\begin{table}[]
\setlength{\lightrulewidth}{0.01em}
\setlength{\cmidrulewidth}{0.01em}
\setlength\tabcolsep{3pt}
\resizebox{1\columnwidth}{!}{
\begin{tabular}{lcccccc}
\toprule
 & \multicolumn{2}{c}{Class name} & \multicolumn{2}{c}{Cap3D prompt} & \multicolumn{2}{c}{Ours} \\ \cmidrule(lr){2-3}  \cmidrule(lr){4-5}  \cmidrule(lr){6-7} 
                        & FID ($\downarrow$)& KID ($\downarrow$)& FID ($\downarrow$)& KID ($\downarrow$) & FID ($\downarrow$) & KID ($\downarrow$)          \\ \midrule
Class name                    &  10.06       &  3.44     & 47.93         & 17.15        &   9.18   &  3.27       \\
Cap3D prompt                  &  -     &  -    & 24.83        &  10.32      &  8.72      & 2.69   \\ \bottomrule
\end{tabular}}
\caption{\textbf{Prompt Engineering.}}
\label{tab:abl_pro}
\end{table}
